GiveMeLabeledIssues: An Open Source Issue Recommendation System

Developers often struggle to navigate an Open Source Software (OSS) project's issue-tracking system and find a suitable task. Proper issue labeling can aid task selection, but current tools are limited to classifying the issues according to their type (e.g., bug, question, good first issue, feature, etc.). In contrast, this paper presents a tool (GiveMeLabeledIssues) that mines project repositories and labels issues based on the skills required to solve them. We leverage the domain of the APIs involved in the solution (e.g., User Interface (UI), Test, Databases (DB), etc.) as a proxy for the required skills. GiveMeLabeledIssues facilitates matching developers' skills to tasks, reducing the burden on project maintainers. The tool obtained a precision of 83.9% when predicting the API domains involved in the issues. The replication package contains instructions on executing the tool and including new projects. A demo video is available at https://www.youtube.com/watch?v=ic2quUue7i8

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> notused.tex <==
\begin{table}[ht!]
 \centering
 \caption{overall metrics from models created to evaluate the corpus. Hla* }
 \label{tab:resultsTFIDF-BERT}
 \begin{tabular}{c|c|c|r|r|r|r} 
  \hline

  \textbf{Model} & \textbf{One/All projects} & \textbf{Precision} & \textbf{Recall} & \textbf{F-measure} &
  \textbf{Hla} \\
  \hline

TD-IDF & S
%&	0.663 &	0.606 &	0.630 &	0.172 \\
%& 0.751 &	0.738 &	0.744 & 0.145\\
& 0.839 & 	0.799 & 	0.817 & 0.113\\

BERT & S
%&	0.663 &	0.606 &	0.630 &	0.172 \\
%& 0.751 &	0.738 &	0.744 & 0.145\\
& 0.595 & 	0.559 & 	0.568 & 0.269\\
TF-IDF & A        &	0.153   &	0.785 &	0.573 &	0.659\\
%Bert                &   0.281   &   0.637 & 0.625 & 0.619 \\
%Bert & 0.204	&		0.738 &	0.417 &	0.53\\
BERT & A & 0.219 & 0.725 & 	0.511 & 	0.593 \\
 \hline
\multicolumn{5}{l}{\scriptsize\textit{* Hla - Hamming Loss }}
 \end{tabular}
\end{table}

%\begin{table}[ht!]
% \begin{center}
%\caption{overall metrics from the model created with the all-projects dataset.}
% \label{tab:resultsAllTogether}
% \begin{tabular}{c|r|r|r|r} 
%  \hline

% \textbf{Model} &
%  \textbf{Hla*} & \textbf{Precision} & %\textbf{Recall} & \textbf{F-measure}  \\
%  \hline

%TF-IDF and RandomForest        &	0.153   &	0.785 &	0.573 &	0.659\\
%Bert                &   0.281   &   0.637 & 0.625 & 0.619 \\
%Bert & 0.204	&		0.738 &	0.417 &	0.53\\
%BERT & 0.219 & 0.725 & 	0.511 & 	0.593 %\\
% \hline
%\multicolumn{5}{l}{\scriptsize\textit{* Hla - Hamming Loss }}
%\\
% \end{tabular}
% \end{center}
%\end{table}

%%%%%%%%%%%%%%%%%%%%%%

\section{GiveMeLabeledIssues Architecture}\label{ToolDesc}

\textit{GiveMeLabeledIssues} leverages prediction models trained with closed issues linked with merged pull requests. On top of these models, we built a platform that receives user input and queries the open issues based on the users' skills and desired projects. In the following, we detail the process of building the model, the issue classification process, and the user interface that enables users to get the recommendation. \textit{GiveMeLabeledIssues} is structured in two layers: the frontend web interface\footnote{https://github.com/JoeyV55/GiveMeLabeledIssuesUI} and the backend REST API\footnote{https://github.com/JoeyV55/GiveMeLabeledIssuesAPI}.

\subsection{Model training}

\begin{figure}[!hbt]
 \centering
 \includegraphics[width=.5\textwidth] {model-training.pdf}
 \caption{The Process of Training a Model}
 \label{fig:training}
\end{figure}

In the current implementation, a model must be built for each project using data collected from project issues linked with merged pull requests. The tool maps the issue text data to the APIs used in the source code that solved the issues (Figure \ref{fig:training}). 

\subsubsection{Mining repositories}

We collected 18,482 issues and 3,129 pull requests (PRs) from JabRef, PowerToys, and Audacity projects up to November 2021. We used the GitHub REST API v3 to collect the title, body, comments, closure date, name of the files changed in the PR, and commit messages.

\subsubsection{APIs parsing}
We built a parser to process all source files from the projects to identify the APIs used in the source code affected by each pull request. In total, we found 3,686 different APIs in 3,108 source files. The parser looked for specific commands, i.e., import (Java), using (C\#), and include (C++). The parser identified all classes, including the complete namespace from each import/using/include statement.

\subsubsection{Dataset construction}
We kept only the data from issues linked with merged and closed pull requests since we needed to map issue data to the APIs that are used in the source code files changed to close the issue. To find the links between pull requests and issues, we searched for the symbol \texttt{\#issue\_number} in the pull request title and body and checked the URL associated with each link. We also filtered out issues linked to pull requests without at least one source code file (e.g., those associated only with documentation files) since they do not provide the model with content related to any API.

\subsubsection{API categorization}
We use the API domain categories defined by \citet{santos2023tell}. These 31 categories were defined by experts to encompass APIs from several projects (e.g., UI, IO, Cloud, DB, etc.---see our replication package\footnote{https://doi.org/10.5281/zenodo.7575116}. 
%After four rounds of discussions ($\approx$ 8 hours), the experts reached a consensus using a card sorting approach and defined 31 API domains. 

%Then, we parsed the APIs found in the commit source code. A similarity function receives a list of API namespaces to determine the possible domains and the percentage of agreement (e.g., sun.oracle.odbc is "DB" with 80\% confidence). The \texttt{spacy} \footnote{https://spacy.io/api/doc\#similarity} python package offers the similarity function, and \texttt{wordninja} \footnote{https://pypi.org/project/wordninja/} package splits the API namespace. Each API received the best API domain found by the similarity function. The experts manually evaluated 100 APIs and approved the categorization in 74.2\% of the cases. 25.8\% were categorized by the experts using card sorting.
%from table 8 (EMSE paper) avg of jabref, audacity and powertoys
%For the TF-IDF model, similar to a previous study \cite{vadlamani2020studying}, we converted each word to lowercase and removed URLs, source code, numbers, and punctuation. After that, we removed templates and stop-words and stemmed the words.

\subsubsection{Corpus construction}
We used the issue title and body as our corpus to train our model since they performed well in our previous analysis~\cite{santos2021can}. Similar to other studies~\cite{behl2014bug,vadlamani2020studying}, we applied TF-IDF as a technique for quantifying word importance in documents by assigning a weight to each word following the same process described in the previous work \cite{santos2021can}. TF-IDF returns a vector whose length is the number of terms used to calculate the scores. Before calculating the scores, we convert each word to lowercase and removed URLs, source code, numbers, and punctuation. After that, we remove templates and stop-words and stem the words. These TF-IDF scores are then passed to the Random Forest classifier (RF) as features for prediction. RF was chosen since it obtained the best results in previous work \cite{santos2021can}. The ground truth has a binary value (0 or 1) for each API domain, indicating whether the corresponding domain is present in the issue solution.

We also offer the option of using a BERT model in \textit{GiveMeLabeledIssues}. We created two separate CSV files to train BERT: an input binary with expert API-domain labels paired with the issue corpus and a list of the possible labels for the specific project. BERT directly labels the issue using the corpus text and lists possible labels without needing an additional classifier (such as Random Forest). 

\subsubsection{Building the model}
The BERT model was built using the Python package fast-bert\footnote{https://github.com/utterworks/fast-bert}, which builds on the Transformers\footnote{\url{https://huggingface.co/docs/transformers/index}} library for Pytorch. Before training the model, the optimal learning rate was computed using a LAMB optimizer~\cite{You2020Large}. Finally, the model was fit over 11 epochs and validated every epoch. The BERT model was trained on an NVIDIA Tesla V100 GPU with an Intel(R) Xeon(R) Gold 6132 CPU within a computing cluster.

TF-IDF and BERT models were trained and validated for every fold in a ShuffleSplit 10-fold cross-validation. Once trained, the models were hosted on the backend. The replication package contains instructions on registering a new project by running the model training pipeline that feeds the demo tool. The models can then output predictions quickly without continually retraining with each request. 
%TF-IDF and BERT were chosen primarily due to previous \cite{santos2021can} and ongoing work that uses them to label issues by API domain.

For the RandomForestClassifier (TF-IDF), the best classifier, we kept the following parameters: criterion = 'entropy,' max depth = 50, min samples leaf = 1, min samples split=3, and n estimators = 50.

\subsection{Issue Classification Process}

\textit{GiveMeLabeledIssues} classifies currently open issues for each registered project. The tool combines the title and body text and sends it to the classifier. The classifier then determines which domain labels are relevant to the gathered issues based on the inputted issue text. The labeled issues are stored in an SQLite database for future requests, recording the issue number, title, body, and domain labels outputted by the classifier.

%\begin{itemize}
 % \item The issue number
% \item The issue title and body text
% \item All the domain labels output by the classifier
%\end{itemize}

The open issues for all projects registered with \textit{GiveMeLabeledIssues} are reclassified daily to ensure that the database is up to date as issues are opened and closed. Figure \ref{fig:Classify} outlines the daily classification procedure. 

\begin{figure}[!hbt]
 \centering
 \includegraphics[width=.5\textwidth] {ClassifySteps.png}
 \caption{The Process of Classifying and Storing Issues}
 %\vspace{-10pt}
 \label{fig:Classify}
\end{figure}


\subsection{User Interface}

\textit{GiveMeLabeledIssues} outputs the labeled issues to the User Interface. The user interface is implemented using the Angular web framework. To use the tool, users provide the project name and select API-domain labels they are interested in. %the following to the front end.
%\begin{enumerate}
% \item The name of the project they would like to work on (selected from a list of projects already classified)
% \item The skills they have (User Interface, Databases, Machine Learning, etc.)
%\end{enumerate}
This information is sent to the backend REST endpoint via a GET request. The backend processes the request, recommending a set of relevant issues for the user. %The query sends the project name and labels to the backend via a GET request.

The backend REST API is implemented using the Django Rest Framework. It houses the trained TF-IDF and BERT text classification models and provides an interface to the labeled issues. When receiving the request, the backend queries the selected project for issues that match the user's skills. Once the query is completed, the backend returns the labeled issues to the user interface. Each labeled issue includes a link to the open issue page on GitHub and the issue's title, number, and applicable labels. The querying process is shown in Figure \ref{fig:OutputtingSteps}.
%that is available to work on within the selected project. The cards 

\begin{figure}[!h]
 \centering
 \includegraphics[width=.5\textwidth] {QuerySteps.png}
 \caption{The Process of Outputting Issues}
 \label{fig:OutputtingSteps}
 %\vspace{-10pt}
 \end{figure}

Figure~\ref{fig:skillSelect} shows JabRef selected as the project and ``Utility,'' ``Databases,'' ``User Interface,'' and ``Application'' as the API domains provided by the user. Figure~\ref{fig:issueResult} shows the results of this query, which displays all JabRef open issues that match those labels.


\begin{figure}[!hbt]
 \includegraphics [width=.5\textwidth] {skillSelection.png}
 \caption{Selection of a project and API domains}
 \label{fig:skillSelect}
 \end{figure}

%\vspace{-10pt}
 \begin{figure}[!hbt]
 \includegraphics [width=.5\textwidth] {threeIssues.png}
 \caption{Labeled Issues Outputted for JabRef with the Utility, Databases, User Interface, and Application skills Selected}
 \label{fig:issueResult}
 \end{figure}
%\vspace{-13pt}

\section{Evaluation}

%So far, our evaluation has been conducted in the terms of the efficiency of the models. 
We have evaluated the performance of the models used to output API-domain labels using a dataset comprised of %22,318 issues, 3,572 pull requests, 12,887 source code files, and 12,331 APIs parsed from three projects, 
%data from EMSE paper table 6.
18,482 issues, 3,129 PRs, 3,108 source code files, and 3,686 distinct APIs, chosen from active projects and diverse domains: Audacity (C++), PowerToys (C\#), and JabRef (Java).\footnote{The model training replication package is available at \url{https://zenodo.org/record/7726323#.ZA5oy-zMIeY}} 
Audacity is an audio editor, PowerToys is a set of utilities for Windows, and JabRef is an open-source bibliography manager. %and which are part of an experiment conducted in another under evaluation article. %=22231-913 table 6 MSRExt paper =4674-1075 =13107-220 =12772-441 = 3942-206
%We evaluated our approach four projects using both TF-IDF and BERT models. 
Table \ref{tab:resultsTFIDF-BERT} shows the results with Precision, Recall, F-Measure, and Hamming Loss values. %While previous studies use Precision, Recall, and F-Measure as performance indicators \cite{santos2021can}, we added hamming loss that measures the fraction of the wrong labels to the total number of labels. 
We trained models to predict API-domain labels using individual issue datasets from each project and a single dataset that combined the data from all the projects. 

%Due to privacy concerns, the %GiveMeLabeledIssues 
%demo does not allow users to access recommendations for the industry project. Thus, the demo includes only the three Open Source projects: JabRef, PowerToys, and Audacity. 

\begin{table}[]
\centering
 \caption{Overall metrics from models -averages. RF-Random Forest* Hla - Hamming Loss**}
 \label{tab:resultsTFIDF-BERT}
\begin{tabular}{|c|c|c|r|r|r|}
\hline
\begin{tabular}[c]{@{}c@{}}Model \\ averages\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{O}ne/\textbf{M}ulti \\ projects\end{tabular} & Precision & Recall & \begin{tabular}[c]{@{}c@{}}F-meas \\-ure \end{tabular}& Hla** \\ \hline
RF* TF-IDF & O & \textbf{0.839} & 0.799 & 0.817 & \textbf{0.113} \\
BERT & O & 0.595 & 0.559 & 0.568 & 0.269 \\
RF* TF-IDF & M & 0.659 & 0.785 & 0.573 & 0.153 \\
BERT & M & 0.593 & 0.725 & 0.511 & 0.219 \\ 
\citet{izadi2022predicting} & M & 0.796 & 0.776 & 0.766 & NA \\
\citet{kallis2019ticket} & M & 0.832 & \textbf{0.826} & \textbf{0.826} & NA \\
\citet{santos2021can} & O & 0.755 & 0.747 &
0.751 & 0.142 \\
\hline
\end{tabular}
%\vspace{-10pt}
\end{table}



\begin{table}[]
\centering
 \caption{Overall metrics from models - by projects. RF-Random Forest* Hla - Hamming Loss**}
 \label{tab:resultsTFIDF-BERT-projects}
\begin{tabular}{|c|c|c|r|r|r|}
\hline
\begin{tabular}[c]{@{}c@{}}Model \\ by project\end{tabular} & \begin{tabular}[c]{@{}c@{}}Project\end{tabular} & Precision & Recall & \begin{tabular}[c]{@{}c@{}}F-meas \\-ure \end{tabular}& Hla** \\ \hline
RF* TF-IDF & Audacity	&\textbf{0.872}	&\textbf{0.839}	&\textbf{0.854} & 0.103\\	
RF* TF-IDF & JabRef	&0.806	&0.782	&0.793 & 0.143\\	
RF* TF-IDF & PowerToys	&0.84	&0.776	&0.805 &\textbf{0.094}\\	
BERT & Audacity		&0.382	&0.511	&0.434 & 0.42\\	
BERT & JabRef	&0.791	&0.606	&0.686	& 0.192\\
BERT & PowerToys	&0.619	&0.643	&0.626 & 0.187\\	
\hline
\end{tabular}
%\vspace{-20pt}
\end{table}

As shown in Table~\ref{tab:resultsTFIDF-BERT}, TF-IDF overcame BERT both in the per-project analysis and for the complete dataset. The difference was quite large when using single projects. The results were closer when we used the combined dataset that included data from all projects (3,736 linked issues and pull requests). We hypothesize that the sample size influenced the classifiers' performance. This aligns with previous research on issue labeling that showed that BERT performed better than other language models for datasets larger than 5,000 issues \cite{wang2021well}. TF-IDF performs very well when the dataset is from a single project because the vocabulary used in the project is very contextual, and the frequency of terms can identify different aspects of each issue. When we include the dataset from all the projects, the performance of TF-IDF drops as the context is not unique. These results outperformed the results from the API-domain labels case study conducted by Santos et al. \cite{santos2021can}. 
%While \citet{kallis2019ticket} results for recall and F-measure overcame all the compared studies, they are limited to "bug", "enhancement", and "question" classification and the feature space with only three possible labels may benefit the approach. In comparison, our models predict many more labels, with PowerToys predicting 13 labels, Jabref 12, and Audacity 20. 
The project metrics (Table \ref{tab:resultsTFIDF-BERT-projects}) varied less than 6\% (e.g., the recall: 0.839 (Audacity) - 0.776 (PowerToys). Audacity had the best scores for all metrics except Hamming Loss. 
